Controlled Power System Separation Using Generator PMU Data and System Kinetic Energy

With the growing number of severe system disturbances and blackouts around the world, controlled system separation is becoming an increasingly important system integrity protection scheme (SIPS) to save the electric power system from a complete or partial disintegration. A successful controlled splitting approach should at least tackle the following two well-known and interrelated problems: "when to split?" and "where to split?". Multiple previous publications consider these problems separately, and even those pursuing a combined approach propose solutions with limited applicability. In this paper, we are proposing a novel PMU-based detector of loss of synchronism that utilizes generator rotor angles and speeds to promptly detect rotor angle instabilities over a wide area. Moreover, we are showing how our loss of synchronism detection principle can be coupled with the known controlled splitting techniques to form an integrated defense scheme against unintentional loss of synchronism. The performance of this wide-area SIPS is demonstrated on the IEEE 39-bus test power system for various types of unstable conditions.

==> issues <==
01) formula (5) is not academic enough: we are using discrete derivatives, what is Delta t and how to express the time window...
02) Linear speed prediction into the future is appropriate: 3-sample linear interpolation for 3-4 PMU samples forward. Simple linear interpolation is crucial as it cannot predict a speed acceleration decrease. Thus it is mostly pessimistic (worst-case), and only if speed starts to go parabolic it may be slightly opimistic (therefore, no more than 3-4 samples forward!)
03) 2-way splitting and IEEE 39 bus in the abstract/intro
04) Cite Matija for coherency
06) A Table with protection parameters (may be later)
07) Change picture Fig. 1!! --> add FINAL equation numbers instead of logic
08) Diagram with group selection distances for various CGGs
09) CGGs for IEEE39 (numbered if possible)
10) In this paper... - remove all and put into parameters table instead
11) Remove newlines before \begin{equation}
12) For phase portraits - add leq 180 condition for angles (unless speed is decreasing)??? - is it valid???

12) Cite Matija, cite GE Iceland
14) Add the statictics (detection time) about all the disturbances. 
13) In Section V mention that if (14) is the trigger, the COI speeds (xx) may be too small. Then only use (15). If (OOS1) or (OOS2), then (critical machine pair speed eqn) must be suitable. 
15) A big table with results for all faults
16) In Figure 3, reduce size by removing extra x-labels (leave only 1 at the bottom)
17) Check degrees for angles on all ylabels
18) Correlation of angles and speeds, or normalize and set to X and Y -> cosine similarity, or, or, or.... Or use predicted values indeed!
19(!!!)) Check COI rotor angles in RSCAD (are 180-210 angle differences really real??)
20) Add PhC to the cover letter (10 pages)
21) For phase portraits, do not justify them by SIME (when saying to choose delta_arm^PP<delta_arm). Phase portrait angles go to 160 and stay stable... May be even to 179!
22) G5 and G9 are weakly connected! State this! Both a prone to disconnect, and even after splitting.






\begin{comment}

Although this study was based on the standard IEEE 39-bus benchmark system with conventional synchronous generators, 
the extension  of inverter-based renewable generators is 

\red{The group selection mechanism aims to mimic a human operator's group selection logic. For slowly evolving undamped oscillations it could be more appropriate to use the existing techniques such as \cite{Sun.2011}.}

\red{Splitting scenario selection can be extended to more than 2 islands. But smaller islands shall be more coherent, at the expense of lower transmission and generation capacity. Thus, a special care must be taken when 
choosing multiway CGGs}

\red{We do not use any curve fitting techniques for prediction of rotor angles and speeds. In our opinion, the use of high-order polynomials could lead to large prediction errors in some cases: the polynomials may diverge a lot outside of the data they were fitted to.}

\red{As we do not rely on unstable network cutsets (e.g., \cite{Padiyar.2006}), it becomes possible to freely choose the lines to open (introduces an extra degree of freedom) - and without using any prediction techniques the reaction time is comparable with \cite{Padiyar.2006} that is using polynomial fitting. -> to the Introduction!!} 

\red{Even if splitting is awaited till the end to see what actually splits (unstable cutset), this unstable cutset may not contain enough inertia and reserves! And by the time two groups \emph{clearly} split, a third group may start to emerge. And unstable line cutsets can be bad from the power balance point of view. }

Energy and COI-based. This is fundamental to AC power systems regardless of the generation mix. Extensions focused on power systems with renewable generators will follow. 
\red{Planning to extend to renewables -- add later}
We are planning to test our splitting scheme in combination with various techniques for estimation of machine rotor angles and frequencies. Another prospective research avenue is the extension of this work to handle inverter-interfaced renewable generators. 
\end{comment}

